Cholesky factorisation, and intrinsically sparse linear quadratic regulation

We classify a family of matrices of shift operators that can be factorised in a computationally tractable manner with the Cholesky algorithm. Such matrices arise in the linear quadratic regulator problem, and related areas. We use the factorisation to uncover intrinsic sparsity properties in the control laws for transportation problems with an underlying tree structure. This reveals that the optimal control can be applied in a distributed manner that is obscured by standard solution methods.

==> bidirectional-tree-K1.tex <==
K_1 = \begin{bmatrix}
 \boldsymbol{\star} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \\
 \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> bidirectional-tree-K2.tex <==
K_2 = \begin{bmatrix}
 \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> big-tree-K1.tex <==
K_1  = \begin{bmatrix}
 \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> big-tree-K2.tex <==
K_2 = \begin{bmatrix}
 \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> tv-string-K1.tex <==
K_1 = \begin{bmatrix}
 \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \boldsymbol{\star} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \boldsymbol{\star} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> tv-string-K2.tex <==
K_2 = \begin{bmatrix}
 \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> unidirectional-tree-K1.tex <==
K_1 = \begin{bmatrix}
 \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}


==> unidirectional-tree-K2.tex <==
K_2 = \begin{bmatrix}
 \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \textcolor{gray}{0} \\
 \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \textcolor{gray}{0} &  \boldsymbol{\star} &  \boldsymbol{\star} &  \boldsymbol{\star} \end{bmatrix}

